EFFOcc: Learning Efficient Occupancy Networks from Minimal Labels for Autonomous Driving

3D occupancy prediction (3DOcc) is a rapidly rising and challenging perception task in the field of autonomous driving. Existing 3D occupancy networks (OccNets) are both computationally heavy and label-hungry. In terms of model complexity, OccNets are commonly composed of heavy Conv3D modules or transformers at the voxel level. Moreover, OccNets are supervised with expensive large-scale dense voxel labels. Model and data inefficiencies, caused by excessive network parameters and label annotation requirements, severely hinder the onboard deployment of OccNets. This paper proposes an EFFicient Occupancy learning framework, EFFOcc, that targets minimal network complexity and label requirements while achieving state-of-the-art accuracy. We first propose an efficient fusion-based OccNet that only uses simple 2D operators and improves accuracy to the state-of-the-art on three large-scale benchmarks: Occ3D-nuScenes, Occ3D-Waymo, and OpenOccupancy-nuScenes. On the Occ3D-nuScenes benchmark, the fusion-based model with ResNet-18 as the image backbone has 21.35M parameters and achieves 51.49 in terms of mean Intersection over Union (mIoU). Furthermore, we propose a multi-stage occupancy-oriented distillation to efficiently transfer knowledge to vision-only OccNet. Extensive experiments on occupancy benchmarks show state-of-the-art precision for both fusion-based and vision-based OccNets. For the demonstration of learning with limited labels, we achieve 94.38\% of the performance (mIoU = 28.38) of a 100\% labeled vision OccNet (mIoU = 30.07) using the same OccNet trained with only 40\% labeled sequences and distillation from the fusion-based OccNet.

==> sec/6_supply.tex <==
\section{Appendix}
\subsection{More Related Works}
\subsubsection{3D Occupancy Prediction} 
3D occupancy prediction originates from the task of semantic scene completion (SSC)\cite{SemanticKITTI}. Occ3D\cite{Occ3D} release benchmarks on large-scale surround-view datasets nuScenes and Waymo, and OccNet\cite{OccNet_OpenDriveLab} extends the challenge to 3d occupancy and flow. Occupancy networks are generally developed from the extension of the vision bird's-eye view (BEV) networks (e.g. BEVDet\cite{BEVDet} and BEVFormer\cite{BEVFormer}) and the semantic segmentation networks\cite{Mask2Former}. SurroundOcc\cite{SurroundOcc} and OpenOccupancy\cite{OpenOccupancy} extract multi-scale 3D voxel features with transformer merge them through deconvolutional upsampling. Multi-scale features proves better segmentation performance. TPVFormer\cite{TPVFormer} and PointOcc\cite{PointOcc} extends BEV formulation to a triple-view feature transformation. PanoSSC\cite{PanoSSC}, Symphonies\cite{Symphonies}, and OccFormer\cite{OccFormer} propose different mask-based transformer heads for panoptic occupancy segmentation. FB-Occ\cite{FB-BEV} proposes a forward BEV-pooling based view transformation module and a backward BEVformer\cite{BEVformer} based transformation and wins 1st on the occupancy prediction challenge. 


\subsection{Definition of 3D Occupancy Prediction Task}

The occupancy prediction task aims at a semantic 3D occupancy grid with a fixed given perception range and resolution. The sensor information is from surround-view cameras and 360-view LiDAR. Each voxel grid is represented by semantics.


\subsection{Dataset and Benchmarks Introduction}

\textbf{Occ3D-nuScenes} is built upon large-scale public available nuScenes dataset\cite{nuscenes},which is a critical resource for advancing 3D object detection and occupancy technologies. It consists of 700 training scenes, 150 scenes for validation and 150 scenes for test, each meticulously annotated at a key frame rate of 2Hz. The sensor configuration of the ego vehicle is 6 ring cameras with resolution $1600\times900$ and one 32-beam LiDAR on the top roof. There are 17 categories of semantics in occ3d-nuScenes including general object. 

% \textbf{Occupancy flow challenge} is an extended annotation whose resolution and perception range is the same as Occ3D-nuScenes. The new labels provide voxel flow ground-truth for dynamic objects. Note that general object is not included in the occupancy flow challenge.

\textbf{Occ3D-Waymo} is built upon large-scale public available Waymo Open Dataset\cite{waymo}.
The dataset comprises 1,000 sequences for trainval split, among which 798 sequences are allocated for the training set and the remaining 202 sequences are designated for validation. Ground-truth labels are annnotated at 10Hz, which is five times more than nuScenes samples. The sensor configuration of the ego vehicle is 5 ring cameras (The rear of the vehicle is not visible by any camera) with resolution $1920\times1280$ or $1920\times1080$ and five LiDARs (equavalent to high-beam LiDAR) on the top roof. There are 15 categories of semantics in occ3d-waymo including the general object category.

For both datasets, the Occ3D splits the surrounding world into 3D voxel grids with the resolution of $[200,200,16]$. The perception range is $[-40m, -40m, -5m, 40m, 40m, 3m]$. For both datasets, we use a voxel size of $0.4m$ meters for voxelization following the prior works.


\textbf{OpenOccupancy-nuScenes} is also built on nuScenes\cite{nuscenes} dataset and shares the same sensor suite with Occ3D-nuScenes. This benchmark is more challenging than Occ3D-nuScenes in that it requires larger perception range $[-51.2m, -51.2m, -5m, 51.2m, 51.2m, 3m]$ and finer resolution $[512,512,40]$ and the voxel size is $0.2m$. A slight difference regarding semantic categories is that OpenOccupancy ignore general object and only has $16$ semantic categories.

\textbf{Metrics for 3D occupancy prediction.} We adopt the official evaluation protocol from CVPR2023 Occupancy Prediction Challenge\footnote{\url{https://opendrivelab.com/challenge2023/#3d_occupancy_prediction}}. We evaluate Intersection-over-Union (IoU) metric over categories and mean IoU. OpenOccupancy also evaluates geometric IoU of occupied voxels as one of the primary metrics. Let $C$ be the number of classes,where $TP_c$ , $FP_c$ and $FN_c$ correspond to the number of true positive, false positive, and false negative predictions for class $c_i$.
\begin{equation}
    mIoU=\frac{1}{C} \sum_{c=1}^{C} \frac{T P_{c}}{T P_{c}+F P_{c}+F N_{c}}
\end{equation}

% \textbf{Metrics for 3D occupancy and flow challenge.} We adopt the official evaluation protocol from CVPR2024 Occupancy and Flow Challenge\footnote{\url{https://opendrivelab.com/challenge2024/#occupancy_and_flow}}.We evaluate occ score as primary metrics. It consists of two parts, which are ray-based mIoU, and absolute velocity error for occupancy flow. The final occupancy score is defined to be a weighted sum of mIoU and mAVE. Note that the velocity errors are converted to velocity scores as,
% \begin{equation}
%     OccScore = mIoU \times 0.9 + max(1 - {mAVE}, 0.0) \times 0.1
% \end{equation}


% \subsection{Implementation Details}

% \textbf{Data Pre-processing.}
% For both training and inference phrases, we first load multi-view images with camera parameters, then apply normalization, padding, and multi-scale flipping to each input image for image augmentation. We aggregate multi-sweep LiDAR point clouds and conduct random flipping on point clouds and voxel labels for BEV augmentation. We don't use any test-time augmentation techniques. 

% \textbf{Training and Inference.} We build our upon the MMDetection3D version 1.0.0rc4 \cite{mmdet3d2020}. Most experiments are trained on 8 2080TI GPUs for 24 epochs in a total batch size of 16, with training time less than 24 hours. We use AdamW optimizer with a learning rate of 0.0001 and weight decay 0.01. We use exponantial moving average (EMA) hook for better accuracy. We set batch size as 1 in the inference stage.


\subsection{Runtime Analysis}
We provide runtime statistics and comparison between RadOcc-LC, EFFOcc-R18, and EFFOcc-Swin-B and demonstrate the effectiveness and efficiency of our proposed fusion-based OccNet.
\begin{table*}[t]
        \caption{Complexity and runtime analysis of our EFFOcc and RadOcc-LC. RadOcc statistics are reported from the original paper.}
	\centering
	\tiny{
            \resizebox{\textwidth}{!}{
		\begin{tabular}{l|cccc|cccc} 
			\hline
			Model & Modality & PC backbone & Img backbone & Image Size & Epochs & FPS  & Param & mIoU \\
			\hline
			BEVDetOcc & C & - & Swin-B & 512x1408  & 24 & 1.0 & 125.91M &44.10\\ 
			RadOcc-LC & LC & SECOND+3DCNN & Swin-B & 512x1408  & - & 0.3 & 135.39M  & 49.38\\
   		    EFFOcc(Ours) & LC & SECOND & R18 & 256x704  & 24  & \textbf{5.6} & \textbf{18.66M}  & 49.29\\
		    % EFFOcc(Ours) & LC & SECOND & R18 & 256x704  & 48  & \textbf{5.6} & \textbf{18.66M}  & 49.59\\
                EFFOcc(Ours) & LC & SECOND & Swin-B & 512x1408  & 24 & 1.8 & 108.59M  & \textbf{54.08}\\
			\hline
		\end{tabular}
          }
		% \vspace{-.3cm}
	}

 \label{tab:runtime_analysis}
\end{table*}


\subsection{Visualizations}
We visualize more 3d occupancy prediction results on Occ3D-nuScenes benchmark validation set based on the visualization tools provided by FlashOcc\cite{FlashOcc}. For the sake of rendering speed, we only plot predictions that are within camera visibility mask of each frame.



\begin{figure*}[htbp]
  \centering
  \begin{tabular}{cccc}
    \includegraphics[width=0.45\textwidth]{fig/occnet/Image1.png} &
    % \includegraphics[width=0.5\textwidth]{fig/occnet/Image21.png} \\
    \includegraphics[width=0.45\textwidth]{fig/occnet/Image24.png} \\
    \includegraphics[width=0.45\textwidth]{fig/occnet/Image10.png} &
    \includegraphics[width=0.45\textwidth]{fig/occnet/Image15.png} \\
    % \includegraphics[width=0.5\textwidth]{fig/occnet/Image33.png} \\
    % \includegraphics[width=0.5\textwidth]{fig/occnet/Image42.png} &
    % \includegraphics[width=0.5\textwidth]{fig/occnet/Image55.png} \\
  \end{tabular}
  \caption{Visualizations of occupancy prediction results on Occ3D-nuScenes validation set.}
  \label{fig:my_figure}
\end{figure*}


We visualize 3d occupancy prediction performance on nuScenes validation set as demo videos on \url{https://github.com/synsin0/EFFOcc}.
% We visualize some difficult cases on both datasets to show the qualitative results of our occupancy network in Fig. \ref{occ_vis_nusc} and Fig. \ref{occ_vis_waymo}.
